Upwards Closed Dependencies in Team Semantics

We prove that adding upwards closed first-order dependency atoms to first-order logic with team semantics does not increase its expressive power (with respect to sentences), and that the same remains true if we also add constancy atoms. As a consequence, the negations of functional dependence, conditional independence, inclusion and exclusion atoms can all be added to first-order logic without increasing its expressive power. Furthermore, we define a class of bounded upwards closed dependencies and we prove that unbounded dependencies cannot be defined in terms of bounded ones.

==> eptcsdata.tex <==
\providecommand{\firstpage}{93}
\providecommand{\publicationstatus}{Gabriele Puppis, Tiziano Villa (Eds.): Fourth International\\ Symposium on Games, Automata, Logics and Formal Verification\\
EPTCS 119, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.119.10}{10.4204/EPTCS.119.10}}

